Grassroots Flash: A Payment System for Grassroots Cryptocurrencies

The goal of grassroots cryptocurrencies is to provide a foundation with which local digital economies can emerge independently of each other and of global digital platforms and global cryptocurrencies; can form and grow without initial capital or external credit; can trade with each other; and can gradually merge into a global digital economy. Grassroots cryptocurrencies turn mutual trust into liquidity and thus could be a powerful means for 'banking the unbanked'. Grassroots cryptocurrencies have not been provided yet with a payment system, which is the goal of this paper. Here, we present Grassroots Flash, a payment system for grassroots cryptocurrencies that employs the blocklace -- a DAG-like counterpart of the blockchain data structure. We analyze its security (safety, liveness, and privacy) and efficiency, prove that it is indeed grassroots.

==> multiagent.tex <==


\mypara{A Fault-Resilient Blocklace-Based Implementation}

A correct agent in the Flash payment system maintains a closed blocklace that only increases; initially has an initial block with input UTXOsan;  issues only balanced transactions; and does not equivocate.
An agent \emph{issues a block} by creating a block with its pending payments and pointers to the roots of it local blocklace, adding the block it to its blocklace and sending it to all agents except those known to be faulty. 

\udi{Not sure what to do about the following BPS.  It is a nice and simple formal specification.  But we need some definitions to be understood, and then the proof that the code implements it is informal.  So maybe leave it out/move to appendix?} \andy{I'd leave it out.}

\begin{definition}[BPS:  Blocklace Payment System]\label{definition:protocol-BPS}
The \temph{blocklace payment system} over $P$  is a distributed multiagent transition system $\textit{BPS}=(P,\textit{BX},T,\lambda)$ with transitions $T$  being all $p$-transitions $c\xrightarrow{}c'$, where $p \in P$, $c'_p= c_p \cup \{b\}$ and one of the following holds:
\begin{enumerate}[partopsep=0pt,topsep=0pt,parsep=0pt]
    \item \textbf{Pay}:   $b$ is $p$-block with a balanced transaction that has ratified inputs
    \item \textbf{Receive-$b$}: $b \in c_q\setminus c_p$ for some $q \in P$. 
\end{enumerate}
The liveness condition $\lambda$ partitions the $p$-transitions according to their labels.
\end{definition}

\begin{proposition}
The BPS transition system satisfies:
\begin{itemize}
    \item \textbf{Safety}:  No double-spending (how to formalize it here?)
    \item \textbf{Liveness}:  Every block known to a correct agent will be known to all
\end{itemize}
\end{proposition}
